The Measure Problem in Cosmology

The Hamiltonian structure of general relativity provides a natural canonical measure on the space of all classical universes, i.e., the multiverse. We review this construction and show how one can visualize the measure in terms of a "magnetic flux" of solutions through phase space. Previous studies identified a divergence in the measure, which we observe to be due to the dilatation invariance of flat FRW universes. We show that the divergence is removed if we identify universes which are so flat they cannot be observationally distinguished. The resulting measure is independent of time and of the choice of coordinates on the space of fields. We further show that, for some quantities of interest, the measure is very insensitive to the details of how the identification is made. One such quantity is the probability of inflation in simple scalar field models. We find that, according to our implementation of the canonical measure, the probability for N e-folds of inflation in single-field, slow-roll models is suppressed by of order exp(-3N) and we discuss the implications of this result.

==> arxiv <==
From no-reply@arXiv.org Tue Jan  2 18:45:50 2007
Date: Tue, 2 Jan 2007 13:45:35 -0500
From: send mail ONLY to hep-th <no-reply@arXiv.org>
Reply-To: hep-th@arXiv.org
To: N.G.Turok@damtp.cam.ac.uk, n.g.turok@damtp.cam.ac.uk
Subject: RE: hrep 0609095 0609095r.tar.gz -> 0609095.tar.gz (hep-th/0609095, 62kb)

To verify abstract and postscript, use http://arxiv.org/abs/hep-th/0609095
  PaperId: hep-th/0609095, PaperPassword: 965zc (access no longer password restricted)

Your replacement has been received and used to replace your earlier submission.
Attached below is an exact copy of the permanent abstract file of your paper.
Please note that if your originally put abstract has already appeared in a
daily mailing, then ONLY the Title/Author/Comments/Report-no/Journal-ref fields
will be used to indicate your replacement in the next mailing. 

------------------------------------------------------------------------------
\\
Paper: hep-th/0609095
From: Neil Turok <N.G.Turok@damtp.cam.ac.uk>
Date: Wed, 13 Sep 2006 21:07:13 GMT   (59kb)
Date (revised v2): Tue, 2 Jan 2007 18:45:32 GMT   (62kb)

Title: The Measure Problem in Cosmology
Authors: G.W. Gibbons and Neil Turok
Comments: 22 pages, 6 figures. Revised version with clarifying remarks on
  meaning of adopted measure, extra references and minor typographical
  corrections
\\
  The Hamiltonian structure of general relativity provides a natural canonical
measure on the space of all classical universes, i.e., the multiverse. We
review this construction and show how one can visualize the measure in terms of
a "magnetic flux" of solutions through phase space. Previous studies identified
a divergence in the measure, which we observe to be due to the dilatation
invariance of flat FRW universes. We show that the divergence is removed if we
identify universes which are so flat they cannot be observationally
distinguished. The resulting measure is independent of time and of the choice
of coordinates on the space of fields. We further show that, for some
quantities of interest, the measure is very insensitive to the details of how
the identification is made. One such quantity is the probability of inflation
in simple scalar field models. We find that, according to our implementation of
the canonical measure, the probability for N e-folds of inflation in
single-field, slow-roll models is suppressed by of order exp(-3N) and we
discuss the implications of this result.
\\

Contains:
 0609095v3.tex: 65366 bytes
 hphi.eps: 77090 bytes
 hphiclosed.eps: 65955 bytes
 hphiopen.eps: 85582 bytes
 inf.eps: 191982 bytes
 phia.eps: 29117 bytes
 pphid.eps: 53707 bytes

Stored as: 0609095.tar.gz (62kb)

Warnings:

Author 1: G.W. Gibbons
Author 2: Neil Turok
-> Number of authors = 2

 0609095r.tar: unpacked 7 files from tar file

 Updated existing cross-list to archive astro-ph
 Updated existing cross-list to archive gr-qc


PS files:
 0609095.ps.gz (165kb)

------------------------------------------------------------------------------
Successful submission to the archives can be a significant source of pride
and accomplishment. It entails many serious responsibilities:
if you can't check off on all items below, then you need to replace again.

  ___ The Title/Author fields above are correct.
     ___ The abstract remains complete, correct, and wrapped correctly.
     ___ Capitalization in title correct (we automatically lower case titles
         with excessive use of upper case, but we get some acronyms incorrect
         -- replace with uppercase letters only where they should be).
     ___ The authors are listed in `Firstname Lastname' order.
     ___ any anonymous ftp or http pointers to additional files are given in
         standard url format (e.g. ftp://myhost.domain/path/filename.ext
         or http://mywwwhost.domain/path/filename.html)
     ___ Periods are separated by a space from the end of any URL's
     ___ Any Journal-ref is a complete bibliographic reference to an already
         published version (includes volume and page number info in the case
         of a print journal).
  ___ All comments about why the paper was replaced are in the Comments: field
      (i.e. not parenthetically after the Title:, or only in the abstract),
      and you retained ALL earlier relevant Comments (e.g. number of pages)
  ___ You have included all the files, e.g. figures (the entire previous
      submission has been overwritten).
  ___ The submission can still be retrieved uncorrupted (TRY IT).

Submitters who repeatedly leave errors uncorrected may lose submission
privilege to the archives.

If your abstract is improperly wrapped, note that abstract linefill stops at
whitespace indentation (e.g. a blank line or a line indented with space(s)
denotes a new paragraph,and won't be wrapped).

For further hints, keep reading or see http://arXiv.org/help/ . Guidelines
for a proper title and abstract preparation are given at
http://arXiv.org/help/prep . If you have not already read this, please read
it now to ensure that you have followed the guidelines. It is an abuse of
valuable archive admin time to edit abstracts by hand.

If this is a replacement on the same day as original submittal, it will
not generate a "replaced" listing in the daily title/abstract distribution
(if replaced before the daily deadline of 16:00 US Eastern time [EDT/EST]
Monday through Friday).

Otherwise, a copy of the original day's submission has been archived; and more
generally each version in the full revision history will remain available.

***NOTES***
1) Common sense suggests that `replaced' papers are not immediately
 rerequested so if your intent is to communicate correct research
 it is in your interest to submit a final version in the first place,
 i.e. *avoid premature submissions*.
 If your replaced submission constitutes a new version, it is helpful to
 indicate in the Comments: field (i.e. below Authors: ) how serious is the
 revision (e.g. v2: major conceptual changes, v3: minor grammatical changes,
 etc.),  and include as a commented header in the revised version of the paper
 a guide to the changes for posterity.
 *** Make sure that these changes are in the Comments: field (i.e. after the
     Authors: ) and that your Abstract still appears ***

2) Avoid excessive cross-listings: cross-listings of a paper on archive-x to
 archive-y are intended for subjects of *direct* interest to subscribers of
 archive-y. Those subscribers of archive-y who have peripheral or direct
 interest in the subjects of archive-x are already subscribed to archive-x and
 neither need nor desire multiple receipt of the same abstract. (In particular,
 it is exceedingly unlikely that you could decide what is of direct interest to
 readers of archive-y if you yourself are not an active reader of archive-y.)

